Quantitative model for $^{13}$C tracing applied to citrate production and secretion of prostate epithelial tissue

Healthy human prostate epithelial cells have the unique ability to produce and secrete large amounts of citrate into the lumen of the prostate. Citrate is a Krebs cycle metabolite produced in the condensation reaction between acetyl-CoA and oxaloacetate in the mitochondria of the cell. With the application of $^{13}$C enriched substrates, such as $^{13}$C glucose or pyruvate, to prostate cells or tissues, it is possible to identify the contributions of different metabolic pathways to this production and secretion of citrate. In this work we present a quantitative model describing the mitochondrial production and the secretion of citrate by prostatic epithelial cells employing the $^{13}$C labeling pattern of secreted citrate as readout. We derived equations for the secretion fraction of citrate and the contribution of pyruvate dehydrogenase complex (PDC) versus the anaplerotic pyruvate carboxylase (PC) pathways in supplying the Krebs cycle with carbons from pyruvate for the production of citrate. These measures are independent of initial $^{13}$C-enrichment of the administered supplements and of $^{13}$C J-coupling patterns, making this method robust also if SNR is low. We propose use of these equations to distinguish between citrate metabolism in healthy and diseased prostate tissue, in particular upon malignant transformation.

==> p09_Figures.tex <==
\section{Figures}
In this section all figures are shown with their captions.\\

==> p11_References.tex <==
% \renewcommand*{\bibfont}{\scriptsize\singlespacing}
\printbibliography
